Minimax Optimal Clustering of Bipartite Graphs with a Generalized Power Method

Clustering bipartite graphs is a fundamental task in network analysis. In the high-dimensional regime where the number of rows $n_1$ and the number of columns $n_2$ of the associated adjacency matrix are of different order, existing methods derived from the ones used for symmetric graphs can come with sub-optimal guarantees. Due to increasing number of applications for bipartite graphs in the high dimensional regime, it is of fundamental importance to design optimal algorithms for this setting. The recent work of Ndaoud et al. (2022) improves the existing upper-bound for the misclustering rate in the special case where the columns (resp. rows) can be partitioned into $L = 2$ (resp. $K = 2$) communities. Unfortunately, their algorithm cannot be extended to the more general setting where $K \neq L \geq 2$. We overcome this limitation by introducing a new algorithm based on the power method. We derive conditions for exact recovery in the general setting where $K \neq L \geq 2$, and show that it recovers the result in Ndaoud et al. (2022). We also derive a minimax lower bound on the misclustering error when $K = L$ under a symmetric version of our model, which matches the corresponding upper bound up to a factor depending on $K$.

==> minimax_old.tex <==
\section{Minimax lower bound}
%\gb{This is a work in progress section, you can skip it for the moment.}
Let us denote  the admissible parameters space by
 \begin{align*}
     \Theta = \lbrace & P\in [0,1]^{n_1\times n_2}: P=Z_1\Pi Z_2^\top \text{ where }\Pi = q\indic_{K}\indic_{K}^\top +(p-q)I_K, 1>p>0,\\
     & q=cp \text{ for some constant }c\in (0,1), Z_1 \in \calM_{n_1,K}, Z_1 \in \calM_{n_2,K} \text{ with } \alpha=1+O\left(\sqrt{\frac{\log n_1}{n_1}}\right) \rbrace.
\end{align*}
 
 %Here $\calM'_{n_1,K}$ (resp. $\calM'_{n_2,K}$) is the subset of $\calM_{n_1,K}$ (resp $\calM_{n_2,K}$) such that Assumption \ref{ass:balanced_part} is satisfied with $\alpha=1+o(1)$. \hemant{I think the symbols $\calM'_{n_1,K}$, $\calM'_{n_2,K}$ do not need to be defined, we can add $\alpha = 1+o(1)$ in the definition of $\Theta$.}

 
 We want to lower bound $\inf_{\hat{z}} \sup_{\theta \in \Theta} \expec (r(\hat{z},z))$ where $\hat{z}$ is an estimator of $Z_1$. For simplicity, we will assume that $K=2$, but we believe that the same argument can be extended to SBiSBM with an arbitrary number of communities $K$. In the supervised case, i.e. when $Z_2$ is known, we can use the same strategy as the one use for the degree-corrected SBM by \cite{dcsbmgao2016} and obtain a lower bound of the order $e^{-(1+o(1))n_2(p-q)/2}$ corresponding to the failure probability of the optimal test associated to the following two hypothesis problem 
 %
 \begin{align*}
     H_0:& G \sim \otimes_{i=1}^{n_2/2} \mathcal{B}(p) \otimes_{i=n_2/2+1}^{n_2} \mathcal{B}(q), \text{ vs}\\
     H_1:& G \sim \otimes_{i=1}^{n_2/2} \mathcal{B}(q) \otimes_{i=n_2/2+1}^{n_2} \mathcal{B}(p).
 \end{align*}  
 %
 However when $n_2\gg n_1\log n_1$ the error associated with this hypothesis testing problem is of order $\exp(-n_2(p-q)/2) \approx \exp(-\sqrt{\frac{n_2\log n_1}{n_1}})$ but this is far smaller than $\exp(-n_1n_2p_{max}^2)$, the misclustering rate obtained for our algorithm. 
 %\hemant{This is not clear, needs to be written more clearly.}.
 A similar phenomena appears for high-dimensional Gaussian mixture models. Indeed, as shown in \cite{Ndaoud2018SharpOR}, it is essential to capture the hardness of estimating the model parameters in the minimax lower bound in order to get the right rate of convergence. The argument developed for obtaining a lower bound of the minimax risk in \cite{Ndaoud2018SharpOR} relies heavily on the Gaussian assumption (they set a Gaussian prior on the model parameters and use the fact that the posterior distribution is also Gaussian) and cannot directly be extended to this setting. 
 
 Our lower bound result is summarised in the following theorem.
 %
  \begin{theorem}\label{thm:minimax} 
  Suppose that $A \sim SBiSBM(Z_1, Z_2, p, q)$ with $K=L=2$,  $n_2\gg n_1 \log n_1$, $n_1n_2p_{max}^2\to \infty$ and $n_1n_2p_{max}^2=O( \log n_1$).
  % $n_1 n_2p_{max}^2 = \Theta(\log n_1)$, 
  %and $\sqrt{n_1\log n_1}n_2p_{max}^2\to 0$,
  Then there exists a constant $c > 0$ such that \[ \inf_{\hat{z}} \sup_{\theta \in \Theta} \expec (r(\hat{z},z)) \geq \exp(-cn_1n_2p_{max}^2) \] where the infimum is taken over all measurable functions $\hat{z}$ of $A$. 
  %If $n_1n_2p_{max}^2=\Theta(1)$, then $\inf_{\hat{z}} \sup_{\theta \in \Theta} \expec (r(\hat{z},z)) \geq c'$ for some positive constant $c'$. 
  
  %\hemant{ I am using $SBiSBM(Z_1, Z_2, p, q)$, is this consistent with earlier notation? Made edits in the statement of the theorem, check. Also, do you mean $n_1n_2p_{max}^2=O(1)$ or $n_1n_2p_{max}^2=\Theta(1)$? Need to be precise in the use of $O$ and $\Theta$ symbols everywhere. Also, don't we need some condition on $n_2 \gg n_1 \log n_1$ somewhere?}
\end{theorem}
%
\begin{remark}
This lower-bound shows that the rate of convergence of our estimator is optimal up to a constant factor. Indeed, for exact recovery, the minimax lower bound implies that $n_1n_2p_{max}^2 \gtrsim \log n_1$ is necessary, while for weak recovery, we need $n_1n_2p_{max}^2\to \infty$.
\end{remark}

%\hemant{I think we need to be precise in the use of asymptotic notation ($\Omega, O, \Theta$ etc.) and non-asymptotic notation ($\gtrsim, \lesssim, \asymp$) throughout the paper. }

\begin{remark}
For simplicity, we only write the proof for $K=L=2$ but we believe it can be extended to the case $ K = L>2$ by reducing the problem to test between two fixed communities as in \cite{dcsbmgao2016}. 
%\hemant{Is it straightforward, or do you ``believe'' it can be extended, as mentioned in the opening paragraphs? Need to be consistent with the language. And what about $K \neq L$?} 
\end{remark}

\begin{proof} The general idea of the proof is to first lower bound the minimax risk by an error occuring in a two hypothesis testing problem and then to replace this hypothesis testing problem by a simpler one. The steps are detailed below.

 \paragraph{Step 1.}
Recall that $z, z'$ denote the partition functions associated with $Z_1$ and $Z_2$ respectively.
 Let $\pi=\pi_1\times \pi_2$ a prior on $(z,\zz)$ such that its marginal on $z$ is sign invariant. By using standard arguments (see \cite{dcsbmgao2016} or \cite{Ndaoud2018SharpOR}) one can show that \[ \inf_{\hat{z}} \sup_{\theta \in \Theta} \expec (r(\hat{z},z)) \gtrsim \frac{2}{n_1}\sum_{i=1}^{\ceil{n_1/2}} \inf_{\hat{z_i}} \expec_\pi \expec( \indic_{\hat{z_i}\neq z_i}| z,\zz)\] where $\hat{z}$ is a measurable function in $A$. %\hemant{$2/n_1$ should be $1/n_1$? since $2$ is hidden as constant? Also, $n_1/2$ not necessarily an integer} Without lost of generality, we can always assume that $\hat{z}_i \in [-1,1]$. \hemant{where do you need $[-1,1]$ later? Also check above inequality once from paper.}
 
 \paragraph{ Step 2.} 
% Without loss of generality, we can assume that $n_2$ is odd (else just delete one column: it won't increase the error).
 We choose as a prior on $z$ and $z'$ a product of independent, centered Rademacher distributions. 
We can write  \[ \expec_\pi \expec( \indic_{\hat{z_i}\neq z_i}| z,\zz) = \expec_{z_{-i}}\expec_{z_i} \expec_{\zz} \expec( \indic_{\hat{z_i}\neq z_i}| z,\zz)\] where $z_{-i}:=(z_j)_{j\neq i}$ and $\expec_X$ means that we integrate only over the random variable $X$. Since $z'$ is random, the entries of $A$ are no longer independent (this is the reason why we use an uninformative prior on $\zz$). 
%\gb{I erased by mistake your comment here. As far as I remember you wanted more explanations for the following fact.}
Note that the quantity $\expec_{\zz} \expec( \indic_{\hat{z_i}\neq z_i}| z,\zz)$ only depends\footnote{Indeed, denoting $\phi_i(A) = \indic_{\hat{z}_i\neq z_i}$, we have $\expec_{\zz} \expec( \indic_{\hat{z}_i\neq z_i}| z,\zz) = \expec_{\zz}\expec[\phi_i(A)|z,\zz] = \expec[\phi_i(A)|z]$.} on $f(A|z)$ the density of $A$ conditionally on $z$. Since the columns of $A$ are independent conditionally on $z$ (because $(\zz_{j})_{j=1}^{n_2}$ are independent) we have that $$f(A|z) = \prod_j f(A_{:j}|z)$$ i.e., $f(A|z)$ is the product of the densities of the columns $A_{:j}$ conditionally on $z$. Now for each $j$ we can write \[ f(A_{:j}|z) = f(A_{ij}|(A_{i'j})_{i'\neq i},z) f((A_{i'j})_{i'\neq i}|z). \] Since $(A_{i'j})_{i'\neq i}$ doesn't depend on $z_i$ we have $f((A_{i'j})_{i'\neq i}|z)= f((A_{i'j})_{i'\neq i}|z_{-i})$. Assume that $z_i=1$. Then $A_{ij} \sim \mathcal{B}(p)$ if $\zz_{j}=1$ or $A_{ij} \sim \mathcal{B}(q)$ if $\zz_{j}=-1$. 
This in turn implies 
\begin{align*} 
\prob (A_{ij}=1|(A_{i'j})_{i'\neq i},z)
&= p \prob(\zz_{j}=1 |(A_{i'j})_{i'\neq i},z )+q\prob(\zz_{j}=-1 |(A_{i'j})_{i'\neq i},z ) \\
%
&= p \prob(\zz_{j}=1 |(A_{i'j})_{i'\neq i},z_{-i} )+q\prob(\zz_{j}=-1 |(A_{i'j})_{i'\neq i}, z_{-i})
\end{align*}
%
Let us denote by $\alpha_j$ the random variable $\prob(\zz_{j}=1 |(A_{i'j})_{i'\neq i},z_{-i} )$. When $z_i = -1$, similar considerations imply 
%
\begin{align*} 
\prob (A_{ij}=0|(A_{i'j})_{i'\neq i},z_{-i})
= q \alpha_j + p (1-\alpha_j).
\end{align*}
%
%
We can write \begin{align}
    \expec_{z_i} \expec_{\zz} \expec( \indic_{\hat{z_i}\neq z_i}| z,\zz) &= \int_{z_i}\int_A \phi_i(A)\prod_j f(A_{ij}|(A_{i'j})_{i'\neq i},z) f((A_{i'j})_{i'\neq i}|z_{-i})\mathrm{d}A\mathrm{d}z_{i}\nonumber\\
    &= \int_{(A_{i'j})_{i'\neq i}}\prod_j f((A_{i'j})_{i'\neq i}|z_{-i}) \underbrace{\left(\int_{z_i}\int_{A_{i:}}\phi_i(A)\prod_jf(A_{ij}|(A_{i'j})_{i'\neq i},z) \mathrm{d}A_{i:}\mathrm{d}z_{i}\right)}_{R_1}\mathrm{d}(A_{i'j})_{i'\neq i}.\label{eq:lowtmp1}
\end{align}

The term $R_1$ corresponds to the risk %$\frac{1}{2}(\inf_\phi \prob_{H_0} \phi +\prob_{H_1} (1-\phi)) $ 
%\hemant{there is a $1/2$ missing inside $\inf$?}
associated with the following two hypothesis testing problem (conditionally on $(A_{i'j})_{i'\neq i}$ and $z_{-i}$)
%
\begin{align*}
     H_0:& G \sim \otimes_{j=1}^{n_2} (\alpha_j\mathcal{B}(p)+(1-\alpha_j)\mathcal{B}(q)) , \text{ vs}\\
     H_1:& G \sim \otimes_{j=1}^{n_2} (\alpha_j\mathcal{B}(q)+(1-\alpha_j)\mathcal{B}(p)).
\end{align*}  
%
%\hemant{In the above test, shouldn't the factor $\prod_j f((A_{i'j})_{i'\neq i}|z_{-i})$ appear for both $H_0, H_1$? If not, why?}
%\gb{ This is a consequence of Neyman Pearson lemma: the minimum error risk is attained for the likelihood ratio statistic and the common factor is cancelled out, so the error is the same as the one associated with the test between $H_0'$ and $H_1'$. }

Unfortunately, for this testing problem, it is difficult to obtain a simplified expression of the optimal test given by the Neyman-Pearson lemma. Our goal is to replace this complex two-hypothesis testing problem by a simpler hypothesis test associated with a smaller error. The proof strategy is the following. When $\alpha_j$ is very close to $1/2$ it is not possible to statistically distinguish $(\alpha_j\mathcal{B}(p)+(1-\alpha_j)\mathcal{B}(q))$ from $(\alpha_j\mathcal{B}(q)+(1-\alpha_j)\mathcal{B}(p))$ and these factors can be dropped. When $\alpha_j>1/2$ we can replace the testing problem $(\alpha_j\mathcal{B}(p)+(1-\alpha_j)\mathcal{B}(q))$ vs $(\alpha_j\mathcal{B}(q)+(1-\alpha_j)\mathcal{B}(p))$ by the simpler testing problem $\mathcal{B}(p)$ vs $\mathcal{B}(q)$ and do a similar simplification when $\alpha_j <1/2$. It remains to control the number of indices for which $\alpha_j>1/2$ and $\alpha_j < 1/2$. It will be shown that they both have the same order $n_2 n_1 p$. Consequently, we would have obtained \[ \inf_\psi \prob_{H_0} \psi +\prob_{H_1} (1-\psi) \gtrsim \inf_\psi \prob_{H'_0} \psi +\prob_{H'_1} (1-\psi)\] where the infimum is taken over all functions $\psi$ measurable in $A$ and $H'_0, H'_1$ correspond to the ``simpler'' tests 
%
\begin{align*}
     H'_0: G \sim \otimes_{i=1}^{n_2n_1p} \mathcal{B}(p)  \text{ vs }
     H'_1: G \sim \otimes_{i=1}^{n_2n_1p} \mathcal{B}(q).
 \end{align*} 
%
It is well known that the error associated with the above testing problem is of the order $e^{-cn_2n_1p^2}$ (see e.g. \cite{dcsbmgao2016}) %\hemant{Give citation}
which corresponds to the rate of convergence of our algorithm. Let us now formalize the above argument.

\paragraph{Step 3.} In order to obtain a lower bound on the risk associated with the two hypothesis testing $H_0$ vs $H_1$ we will need to condition on several events $\calE_1,\ldots, \calE_4$ occurring with high probability that will be defined later. Since we integrate over non negative quantities, we obtain using \eqref{eq:lowtmp1} 
\begin{align}
     &\expec_{z_{-i}}\expec_{z_i}  \expec( \indic_{\hat{z_i}\neq z_i}| z) \geq \nonumber\\ &\int_{z_{-i}}\indic_{\calE_1}\int_{(A_{i'j})_{i'\neq i}}\indic_{\calE_2\cap \calE_3}\prod_j f((A_{i'j})_{i'\neq i}|z_{-i}) \left(\int_{z_i}\int_{A_{i:}}\indic_{\calE_4}\phi_i(A)\prod_jf(A_{ij}|(A_{i'j})_{i'\neq i},z) \mathrm{d}A_{i:}\mathrm{d}z_{i}\right)\mathrm{d}(A_{i'j})_{i'\neq i}\mathrm{d}z_{-i} \label{eq:lb_cond}
\end{align}


\paragraph{Step 4.} First, we will study under what conditions $\alpha_j \approx 1/2$.
 A simple calculation shows that \[ \frac{\alpha_j}{1-\alpha_j}= \frac{\prod_{i' \neq i: z_{i'}=1}p^{A_{i'j}}(1-p)^{1-A_{i'j}} \prod_{i' \neq i: z_{i'}=-1}q^{A_{i'j}}(1-q)^{1-A_{i'j}} }{\prod_{i' \neq i: z_{i'}=1}q^{A_{i'j}}(1-q)^{1-A_{i'j}} \prod_{i' \neq i: z_{i'}=-1}p^{A_{i'j}}(1-p)^{1-A_{i'j}}}:=\theta_j.
 \]
Let us denote by $\calC_+$ (resp $\calC_-$) the set $\lbrace i' \neq i: z_{i'}=+1 \rbrace$ (resp. $\lbrace i' \neq i: z_{i'}=-1 \rbrace$ ). Then the previous expression can be rewritten as \[ \theta_j = \left(\frac{p(1-q)}{q(1-p)}\right)^{\sum_{i'\in \calC_+}A_{i'j}-\sum_{i'\in \calC_-}A_{i'j}}\left(\frac{1-p}{1-q}\right)^{|\calC_+|-|\calC_-|} .\]  We also have the relation $\alpha_j = \frac{\theta_j}{1+\theta_j}$, so $\alpha_j$ is close to $1/2$ if and only if $\theta_j$ is close to $1$. If $z_{-i}$ were an exactly balanced partition, i.e., $|\calC_+|-|\calC_-|=0$, then $\theta_j=1$ would be equivalent to $\sum_{i'\in \calC_+}A_{i'j}-\sum_{i'\in \calC_-}A_{i'j}=0$. Unfortunately when the communities are generated with independent Rademacher, the size of the resulting communities are rarely exactly the same. 
%\hemant{you mean $z_{-i}$ is not balanced?} 
However the contribution of the term $\left(\frac{1-p}{1-q}\right)^{|\calC_+|-|\calC_-|}$ is small because it is very close to $1$ w.h.p. Indeed, we have $|\calC_+|-|\calC_-|\in [-C\sqrt{n_1\log n_1}, C\sqrt{n_1 \log n_1}]$ for some positive constant $C>0$ with probability at least $1-n_1^{-c}$ for some positive constant $c$ by Hoeffding's inequality that can be choosen arbitrary large depending on the choice of $C$. Let us denote this event by  \begin{align}
    \calE_1 =\left\lbrace z_{-i}:  |\calC_+|-|\calC_-|\in [-C\sqrt{n_1\log n_1}, C\sqrt{n_1 \log n_1}]\right\rbrace.
\end{align} We will condition on this event that is independent from $z_i$ and $A$ (it only depends on $z_{-i}$). Moreover, note that $\log (\frac{1-p}{1-q})\in [-c(p-q),c(p-q)]$ by using Taylor's formula. Hence,  
\[  
\left(\frac{1-p}{1-q}\right)^{|\calC_+|-|\calC_-|} \in [e^{-c'\sqrt{n_1\log n_1}p},e^{c'\sqrt{n_1\log n_1}p} ]
\] 
for some positive constant $c'>0$. But we have \[ \max (|e^{c'p\sqrt{n_1\log n_1}}-1|,|e^{-c'p\sqrt{n_1\log n_1}}-1|)\leq c'p\sqrt{n_1\log n_1}:= \epsilon .\] Therefore, it follows that  $(\frac{1-p}{1-q})^{|\calC_+|-|\calC_-|} \in [1-\epsilon , 1+ \epsilon]$ w.h.p.


On the other hand when $\sum_{i'\in \calC_+}A_{i'j}-\sum_{i'\in \calC_-}A_{i'j}\neq 0$ the quantity $\left(\frac{p(1-q)}{q(1-p)}\right)^{\sum_{i'\in \calC_+}A_{i'j}-\sum_{i'\in \calC_-}A_{i'j}}$ will be at least $p/q>1$ or at most $q/p<1$. This implies that the information provided by the size of the partition will only matter in the decision process when $\sum_{i'\in \calC_+}A_{i'j}-\sum_{i'\in \calC_-}A_{i'j} = 0$. But since it provides very little information, it can be disregarded as will be shown in the next steps.

\paragraph{Step 5.} We need to control the size of the set $j\in [n_2]$ for which $\theta_j\in [1-\epsilon, 1+\epsilon]$. Conditionally on $\calE_1$, it can only happen for the indices $j$ such that $\sum_{i'\in \calC_+}A_{i'j}-\sum_{i'\in \calC_-}A_{i'j}= 0$. But this last event occurs with probability at least $(1-p)^{n_1-1} = 1-\Theta(n_1p)$ (the probability that all the $A_{i'j}$ are simultaneously null). To obtain an upper bound of this probablity, we can use Paley-Zigmund inequality as follows. Let us denote $Z=|\sum_{i'\in \calC_+}A_{i'j}-\sum_{i'\in \calC_-}A_{i'j}|$. We have \[ \prob (Z=0)=1-\prob(Z>0)\leq 1- \prob(Z>\theta \expec Z) \leq 1-(1-\theta)^2\frac{\expec( Z)^2}{\expec (Z^2)}\] for a $\theta \in (0,1)$ by Paley-Zigmund inequality. It is easy to check that $\expec Z\gtrsim n_1(p-q)$ and $\expec(Z^2)\asymp n_1p$. Consequently, $\prob(Z=0)\leq 1-Cn_1p$ for some constant $C>0$.

But by Chernoff's multiplicative bound we have that \[ \sum_j \indic_{\lbrace \sum_{i'\in \calC_+}A_{i'j}-\sum_{i'\in \calC_-}A_{i'j}\neq 0 \rbrace} = \Theta( n_2n_1p)\] with probability at least $1-e^{-cn_2n_1p}$, for any realization of $z_{-i}$. Notice that this event is independent of $A_{i:}$ and $z_i$. Let us denote denote this event by \begin{equation}\label{eq:def_e2}
    \calE_2 =\left\lbrace  \sum_j \indic_{\lbrace \sum_{i'\in \calC_+}A_{i'j}-\sum_{i'\in \calC_-}A_{i'j}\neq 0 \rbrace} = \Theta( n_2n_1p) \right\rbrace
\end{equation} and define  \[ J_b:=\lbrace j\in [n_2] : \theta_j\in [1-\epsilon, 1+\epsilon]\rbrace \] and \[ J_g:=\lbrace j\in [n_2] : \theta_j\notin [1-\epsilon, 1+\epsilon]\rbrace.\] Then conditionally on $\calE_1\cap\calE_2$ we have \[ |J_b|= (1-o(1))n_2, \text{ and } |J_g| =\Theta( n_2n_1p) .\]

\paragraph{Step 6.}It is easy to check  $\theta_j\in [1-\epsilon, 1+\epsilon]$ implies $\alpha_j\in [1/2-\epsilon', 1/2+\epsilon']$ for $\epsilon'$ proportional to $\epsilon$. Since the constant involved here doesn't matter, we won't make a distinction between $\epsilon$ and $\epsilon'$. 

For all $j\in [n_2]$ such that $\alpha_j\in [1/2-\epsilon, 1/2+\epsilon]$ we can check that \[ \alpha_jp^{A_{ij}}(1-p)^{1-A_{ij}}+(1-\alpha_j)q^{A_{ij}}(1-q)^{1-A_{ij}}\geq (1-\epsilon) \frac{p+q}{2}\indic_{A_{ij}=1} + (1-p\epsilon)\frac{1-p+1-q}{2}\indic_{A_{ij}=0}. \]

In particular \scriptsize \[ \prod_{j \in J_b}\alpha_j p^{A_{ij}}(1-p)^{1-A_{ij}}+(1-\alpha_j)q^{A_{ij}}(1-q)^{1-A_{ij}} \geq (1-\epsilon)^{\sum_{j\in J_b}A_{ij}} (1-p\epsilon)^{\sum_{j\in J_b}(1-A_{ij})}\prod_{j \in J_b}\frac{p^{A_{ij}}(1-p)^{1-A_{ij}}+q^{A_{ij}}(1-q)^{1-A_{ij}} }{2}. \]
\normalsize

Let us define the event \begin{equation}\label{eq:def_e4}
    \calE_4=\left\lbrace \sum_{j\in J_b}A_{ij} = \Theta(n_2p) \right\rbrace .
\end{equation}
This event is independent of $(A_{i'j})_{i'\neq i, j}$ and conditionally on $\calE_1\cap \calE_2$, we have for all choice of $z_i$ and $\zz$ that $\prob(\calE_4|\calE_1\cap \calE_2)\geq 1-e^{-cn_2p}$. This implies that conditionally on $\calE_4$ we have  $(1-\epsilon)^{\sum_{j\in J_b}A_{ij}} = 1-\Theta(\sqrt{n_1\log n_1}n_2p^2)$.  We can obtain a similar bound for $(1-p\epsilon)^{\sum_{j\in J_b}(1-A_{ij})}) = 1-\Theta(\sqrt{n_1\log n_1}n_2p^2) $. Since by assumption $\sqrt{n_1\log n_1}n_2p^2 \to 0$, $(1-\epsilon)^{\sum_{j\in J_b}A_{ij}} (1-p\epsilon)^{\sum_{j\in J_b}(1-A_{ij})}=1-o(1)$. This shows that for all $j\in J_b$ we can replace all the factors $(\alpha_j\mathcal{B}(p)+(1-\alpha_j)\mathcal{B}(q))$ by $(\frac{1}{2}\mathcal{B}(p)+\frac{1}{2}\mathcal{B}(q))$ in the hypothesis testing problem and obtain a proportional error. Indeed we have shown that \begin{align*}
    \int_{z_i}\int_{A_{i:}}\indic_{\calE_4}\phi_i(A)\prod_jf(A_{ij}|(A_{i'j})_{i'\neq i},z) \mathrm{d}A_{i:} \geq (1-o(1))\int_{z_i}\int_{A_{i:}}\indic_{\calE_4}\phi_i(A)\prod_{j\in J_g}f(A_{ij}|(A_{i'j})_{i'\neq i},z)\prod_{j\in J_b}g(A_{ij}) \mathrm{d}A_{i:}
\end{align*} where $g$ is the density associated with $(\frac{1}{2}\mathcal{B}(p)+\frac{1}{2}\mathcal{B}(q))$. Since $g$ doesn't depend on $z_i$ \small \[ \int_{z_i}\int_{A_{i:}}\indic_{\calE_4}\phi_i(A)\prod_{j\in J_g}f(A_{ij}|(A_{i'j})_{i'\neq i},z)\prod_{j\in J_b}g(A_{ij}) \mathrm{d}A_{i:} = \int_{(A_{ij})_{j\in J_b}}\prod_{j\in J_b}g(A_{ij})\int_{z_i}\int_{(A_{ij})_{j\in J_g}}\indic_{\calE_4}\phi_i(A)\prod_{j\in J_g}f(A_{ij}|(A_{i'j})_{i'\neq i},z) \] \normalsize

\paragraph{Step 7.} It remains to simplify the testing problem for $j\in J_g$. Let $T_j \sim \calB (\alpha_j)$ be independent Bernoulli with parameter $\alpha_j$. Then \[ \expec_{T_j} (\underbrace{p^{A_{ij}}(1-p)^{A_{ij}}T_j+  q^{A_{ij}}(1-q)^{A_{ij}}(1-T_j)}_{f_{T_j}(A_{ij})})= p^{A_{ij}}(1-p)^{A_{ij}}\alpha_j+  q^{A_{ij}}(1-q)^{A_{ij}}(1-\alpha_j). \] But $T_j$ is independent from $z_i$ and $A_i$, so we can interchange the integration over $T_j$ and $z_i$. It leads to a testing problem  
\begin{align*}
     H''_0:& G \sim \otimes_{T_j=1} \mathcal{B}(p)\otimes_{T_j=0} \mathcal{B}(q) , \text{ vs}\\
     H''_1:& G \sim \otimes_{T_j=1} \mathcal{B}(q)\otimes_{T_j=0} \mathcal{B}(p).
 \end{align*} 
  
Indeed we have \small\begin{align*}
    \int_{z_i}\int_{A_{i:}}\indic_{\calE_4}\phi_i(A)\prod_{j\in J_g}f(A_{ij}|(A_{i'j})_{i'\neq i},z)\prod_{j\in J_b}g(A_{ij}) \mathrm{d}A_{i:}\mathrm{d}z_{i}&= \int_{z_i}\int_{A_{i:}}\indic_{\calE_4}\phi_i(A)\prod_{j\in J_g}\expec_{T_j}f_{T_j}(A_{ij})\prod_{j\in J_b}g(A_{ij}) \mathrm{d}A_{i:}\mathrm{d}z_{i} \\
    &=\expec_{T_j}\int_{z_i}\int_{A_{i:}}\indic_{\calE_4}\phi_i(A)\prod_{j\in J_g}f_{T_j}(A_{ij})\prod_{j\in J_b}g(A_{ij}) \mathrm{d}A_{i:}\mathrm{d}z_{i}\\
    &\geq \expec_{T_j}\int_{z_i}\int_{A_{i:}}\phi_i(A)\prod_{j\in J_g}f_{T_j}(A_{ij})\prod_{j\in J_b}g(A_{ij}) \mathrm{d}A_{i:}\mathrm{d}z_{i}-\prob(\calE_4^c).
\end{align*}  
  \normalsize
 %  Since  $|j : T_j=1| + |j : T_j=0|= |J_g|=\Theta(n_1n_2p_{max})$, the risk of this test is lower bounded by  $e^{-cn_1n_2p^2}$ using Lemma 4 in \cite{dcsbmgao2016}.

\paragraph{Step 8.}
 We need to show that $|j : T_j=1|$ and $|j : T_j=0|$ are approximately equal for a typical realization of $(T_j)_j$. We have 
 $$\expec(|j : T_j=1|)=\sum_{j\in J_g}\alpha_j= \sum_{j\in [n_2]}\alpha_j\indic_{\alpha_j \notin [1/2-\epsilon, 1/2+\epsilon]}$$ and similarly  $$\expec(|j : T_j=0|)=\sum_{j\in [n_2]}(1-\alpha_j)\indic_{\alpha_j \notin [1/2-\epsilon, 1/2+\epsilon]}.$$ Since $\alpha_j$ is almost symmetric around $1/2$ we should have $|j : T_j=1|/|j : T_j=0|=1+o(1)$ w.h.p. We are now going to formalize this argument. Let us define $\tilde{\calC}_+$ and $\tilde{\calC}_-$ by removing elements of the set of maximal size between $\calC_+$ and $\calC_-$ so that $|\tilde{\calC}_+|=|\tilde{\calC}_-|$. Conditionally on $\calE_1$, we have $|\tilde{\calC}_-|=(1-o(1))\frac{n_1}{2}$.
 
 Let us write \[ \Tilde{\alpha_j}:=\alpha_j \indic_{\alpha_j \notin [1/2-\epsilon, 1/2+\epsilon]} = \indic_{\lbrace \sum_{i'\in \calC_+}A_{i'j}-\sum_{i'\in \calC_-}A_{i'j}\neq 0 \rbrace} = \indic_{\lbrace \sum_{i'\in \tilde{\calC}_+}A_{i'j}-\sum_{i'\in \tilde{\calC}_-}A_{i'j} +Z_j\neq 0 \rbrace}\] where we decompose the difference $\sum_{i'\in \calC_+}A_{i'j}-\sum_{i'\in \calC_-}A_{i'j}$ into a difference of independent Bernoulli over exactly balanced sets of size $(1-o(1))n_1/2$ plus an approximation term $Z_j$ that corresponds to the fact that $\calC_+$ and $\calC_-$ are approximately equal. By definition, under $\calE_1$, $Z_j$ is the sum of at most $O(\sqrt{n_1\log n_1})$ Bernoulli r.v. with parameters $p$ or $q$.  Since $|\calC_+|/|\calC_-|=1+O(\sqrt{\frac{\log n_1}{n_1}})$ , by using the same argument as in Step 5., we have  that $Z_j=0$ with probability at least $1-\Theta(\sqrt{n_1\log n_1}p)$. 
 %We also have by concentration inequality that with probability at least $1-e^{-C\log n_1}$ that $|Z_j|\leq $ 
 Let $\alpha_j^* := \indic_{\lbrace \sum_{i'\in \tilde{\calC}_+}A_{i'j}-\sum_{i'\in \tilde{\calC}_-}A_{i'j} \neq 0 \rbrace}$. Since we take sum over exactly balanced sets and $\zz_{j}$ is a Rademacher variable, $\alpha_j^*$ is symmetric around $1/2$. So we have $\expec (\sum_j \Tilde{\alpha_j})= \expec (\sum_j \alpha_j^*)+\Theta(\sqrt{n_1\log n_1}n_2p) $. But since $\alpha_j^* $ are symmetric around $1/2$, \[\expec(\sum_j \alpha_j^*) = \expec(\sum_j (1-\alpha_j^*))=\Theta(n_1n_2p).\] Consequently $\expec(\sum_j \tilde{\alpha}_j)=(1+o(1))\expec(\sum_j \alpha_j^*)$. Let us denote the event \[ \calE_3= \left\lbrace \sum_j\tilde{\alpha}_j =(1-o(1))\expec(\sum_j\tilde{\alpha}_j )  \right\rbrace.\] By using multiplicative Chernoff bound, with $\delta= 1/\sqrt{\log n_1}$,  this event holds with probability at least\footnote{Under our assumptions we have  $p\gtrsim (n_1n_2)^{-1/2}$, hence  $n_1n_2p/\log n_1\gg \log n_1 n_1n_2p_{max}^2$ for $n_1$ large enough.} $1-e^{-\Omega(n_1n_2p/\log n_1)}$, conditionally on $\calE_1$. 
 Finally, let us denote the event \[ \calE_5= \left\lbrace |j : T_j=1|=(1+o(1))|j : T_j=0|=(1+o(1))\expec(\sum_j \alpha_j^*) \right\rbrace. \] This event also holds with probability at least $1-e^{-\Omega(n_1n_2p/\log n_1)}$ conditionally on $\calE_3$, by using the same argument as before.
 
 %By concentration inequality $|j : T_j=1|= \Theta( \sum_{j\in J_g}\alpha_j)$ and $|j : T_j=0|=\Theta( \sum_{j\in J_g}(1-\alpha_j))$ w.h.p. But it is easy to sea that $\prob (\alpha_j>1/2) = \prob (\alpha_j<1/2)$ (because of the choice of the prior on $z_2$) so there are approximately as many indexes $j$ such that $\alpha_j>1/2$ than indexes such that $\alpha_j<1/2$. It implies that all the sums are of order $n_2n_1p$.
  
 \paragraph{Conclusion.} 
 
 By Neyman-Pearson lemma, the quantity \[ \indic_{\calE_5}\int_{z_i}\int_{A_{i:}}\phi_i(A)\prod_{j\in J_g}f_{T_j}(A_{ij}) \mathrm{d}A_{i:}\mathrm{d}z_{i}\] 
 
is lower bounded by the risk associated with the following two hypothesis testing problem (since the 
  \begin{align*}  H'''_0:& G \sim \otimes_{j=1}^{m} \mathcal{B}(p)\otimes_{j=m+1}^{m+m'} \mathcal{B}(q) , \text{ vs}\\ H'''_1:& G \sim \otimes_{j=1}^{m} \mathcal{B}(q)\otimes_{j=m+1}^{m+m'}\mathcal{B}(p).
 \end{align*} 
where $m= |j : T_j=1|, m'= |j : T_j=0|$ and $m/m'=1+o(1)$ since we have conditioned on $\calE_5$.  By the results in Lemma 4 in \cite{dcsbmgao2016}, this risk is lower bounded by $e^{-|j : T_j=1|(p-q)}=e^{-\Theta(n_1n_2p^2)}$. Now to obtain a lower bound on $\expec_\pi \expec( \indic_{\hat{z_i}\neq z_i}| z,\zz)$ it remains to integrate all the events $\calE_i$ we conditioned on. But since they all occur with probability $1-o(1)$ we obtain $e^{-\Theta(n_1n_2p^2)}$ as a lower bound.

%The same argument can be used in the case were $n_1n_2p^2=\Theta(1)$ the only difference is that at the last step the risk associated with the two hypothesis testing problem $H_0'''$ vs $H_1'''$ is lower bounded by an absolute constant.
\end{proof}

